EntropyStop: Unsupervised Deep Outlier Detection with Loss Entropy

Unsupervised Outlier Detection (UOD) is an important data mining task. With the advance of deep learning, deep Outlier Detection (OD) has received broad interest. Most deep UOD models are trained exclusively on clean datasets to learn the distribution of the normal data, which requires huge manual efforts to clean the real-world data if possible. Instead of relying on clean datasets, some approaches directly train and detect on unlabeled contaminated datasets, leading to the need for methods that are robust to such conditions. Ensemble methods emerged as a superior solution to enhance model robustness against contaminated training sets. However, the training time is greatly increased by the ensemble. In this study, we investigate the impact of outliers on the training phase, aiming to halt training on unlabeled contaminated datasets before performance degradation. Initially, we noted that blending normal and anomalous data causes AUC fluctuations, a label-dependent measure of detection accuracy. To circumvent the need for labels, we propose a zero-label entropy metric named Loss Entropy for loss distribution, enabling us to infer optimal stopping points for training without labels. Meanwhile, we theoretically demonstrate negative correlation between entropy metric and the label-based AUC. Based on this, we develop an automated early-stopping algorithm, EntropyStop, which halts training when loss entropy suggests the maximum model detection capability. We conduct extensive experiments on ADBench (including 47 real datasets), and the overall results indicate that AutoEncoder (AE) enhanced by our approach not only achieves better performance than ensemble AEs but also requires under 2\% of training time. Lastly, our proposed metric and early-stopping approach are evaluated on other deep OD models, exhibiting their broad potential applicability.

==> bound_proof.tex <==
\section{Range of Speed Gap under Gradient Descent}

\subsection{Notations}
We summarize here the notations for the derivation of the range:

\begin{itemize}
    \item $\mathcal{D}$ : the dataset.
    \item $\left|C_0\right|$ : the number of samples belonging to inlier class. 
    \item $\left|C_1\right|$ : the number of samples belonging to outlier class. 
    \item $R=\frac{\left|C_0\right|}{\left|C_1\right|}$ : the ratio of the numbers of samples between inliers and outliers.
    \item $L$ : Lipschitz constant, with regard to Lipschitz smooth.
    \item $t$ : time of the training process (i.e., number of iteration).
\end{itemize}
At each time $t$, we have:
\begin{itemize}
    \item $\eta_t$ : learning rate, a positive real number.
    \item $\omega_t$ : set of network parameters.
    \item $f(\omega_t)={\textstyle\sum_{x\in\mathcal{D}}f(x; \omega_t)}$ : loss value summed over all samples in the dataset.
    \item $f^{i}(\omega_t)={\textstyle\sum_{x\in{C_i}}f(x; \omega_t)}$ : loss value summed over all samples belonging to class $i$.
    \item $\nabla f^{i}(\omega_t)$ : gradient computed on the loss function summed over all samples belonging to class $i$.
    \item $\theta_t$ : the angle between $\nabla f^{0}(\omega_t)$ and $\nabla f^{1}(\omega_t)$.
    \item $\nabla f(\omega_t) = \nabla f^{0}(\omega_t) + \nabla f^{1}(\omega_t)$ : gradient computed on the loss function summed over all samples.
    \item $\nabla_{i} = \left\| \nabla f^{i}(\omega_t) \right\|$ : the norm of the overall gradient of class $i$. For clarity, $t$ is omitted in the simplified notation $\nabla_{i}$ in some formulas.
    \item $r_t=\frac{\nabla_{0}}{\nabla_{1}}$ : the ratio of class gradient norms.
    \item ${\triangle}^f_t = \frac{1}{\left|C_0\right|}(f^{0}(\omega_t)-f^{0}(\omega_{t+1}))-\frac{1}{\left|C_1\right|}(f^{1}(\omega_t)-f^{1}(\omega_{t+1}))$: \textit{speed gap}, the difference of the decreasing speed of averaged loss value between two classes.
\end{itemize}

\subsection{Derivation of the range}
In previous proofs, we show that a positive speed gap benefits AUC and lowers loss entropy simultaneously. To provide a further insight of speed gap between inliers and outliers, a range of speed gap is calculated as follows.

In the former part of the derivation, we only detailed the situation of class $i$, since the other one is completely the same.

\begin{assumption}\label{assumption1}
Assume that for each class $i$, $f^i$ is $L-Smooth$.
\end{assumption}
\begin{assumption}\label{assumption2}
At each time $t$, there exists a learning rate $\eta_t>0$ being sufficiently small to guarantee the decrease of both $f^{0}$ and $f^{1}$.
\end{assumption}

% \begin{lemma}
% Assume that for each $l$, $f^{0}(\omega_t)$ is $L-Smooth$.
% \end{lemma}

% \begin{theorem}
% Assume that for each $l$, $f^{0}(\omega_t)$ is $L-Smooth$.
% \end{theorem}

\begin{proof}
In each iteration, gradient descent algorithm use the gradient summed over all samples to update the parameters:
\begin{align}
\omega^{t+1}=\omega^{t}-\eta_t\nabla f(\omega_t) \notag
\end{align}
\noindent Since each $f^{0}(\omega_t)$ is $L-Smooth$, we have
\begin{align}
f^{0}(\omega_{t+1}) &= f^{0}(\omega_t) + \nabla f^{0}(\omega_t)^{\mathrm{T}}(\omega_{t+1} - \omega_{t}) \notag
\\&\qquad\qquad+ \frac{1}{2} (\omega_{t+1} - \omega_{t})^{\mathrm{T}} \nabla^2f(u)(\omega_{t+1} - \omega_{t}) \label{applyTaylor}
\\ &\le f^{0}(\omega_t) + \nabla f^{0}(\omega_t)^{\mathrm{T}}(\omega_{t+1} - \omega_{t}) + \frac{L}{2} \left \| \omega_{t+1} - \omega_{t} \right \| ^2 \label{applySmoothUpper},
\end{align}

\noindent and
\begin{align}
f^{0}(\omega_{t+1}) \ge f^{0}(\omega_t) + \nabla f^{0}(\omega_t)^{\mathrm{T}}(\omega_{t+1} - \omega_{t}) - \frac{L}{2} \left \| \omega_{t+1} - \omega_{t} \right \| ^2 \label{applySmoothLower},
\end{align}

\noindent In \eqref{applyTaylor}, $f(u)$ is some convex combination of $\omega_{t+1}$ and $\omega_{t}$ with respect to multivariate Taylor expansion. We have \eqref{applySmoothUpper} and \eqref{applySmoothLower} by applying Lipschitz smooth, which ensures the term $(\omega_{t+1} - \omega_{t})^{\mathrm{T}} \nabla^2f(u)(\omega_{t+1} - \omega_{t})$ is at most $L \left \| \omega_{t+1} - \omega_{t} \right \| ^2$ and at least $-L \left \| \omega_{t+1} - \omega_{t} \right \|$. We first focus on the upper bound guaranteed by \eqref{applySmoothUpper}.

\begin{align}
f^{0}(\omega_{t+1}) &\le f^{0}(\omega_t) - \eta_t\nabla f^{0}(\omega_t)^{\mathrm{T}}\nabla f(\omega_t) + \frac{\eta_t^2 L}{2} \left \| \nabla f(\omega_t) \right \| ^2 \notag
\\ &= f^{0}(\omega_t) - \eta_t(\left \| \nabla f^{0}(\omega_t) \right \|^2 + \nabla f^{0}(\omega_t)^\mathrm{T}\nabla f^{1}(\omega_t)) \notag
\\ &\qquad\qquad + \frac{\eta_t^2 L}{2} \left \| \nabla f^{0}(\omega_t) + \nabla f^{1}(\omega_t) \right \|^2 \notag
\end{align}
\noindent From this, we can derive a lower bound of the decreasing speed of averaged loss: 
\begin{align}
& \frac{1}{\left|C_0\right|}(f^{0}(\omega_t)-f^{0}(\omega_{t+1})) \ge \notag
\\ &-\frac{\eta_t^2 L}{2\left|C_0\right|} (\left \| \nabla f^{0}(\omega_t) \right \|^2 + \left \| \nabla f^{1}(\omega_t) \right \|^2 + 2\cos{\theta_t}\left \| \nabla f^{0}(\omega_t) \right \| \left \| \nabla f^{1}(\omega_t) \right \|) \notag
\\ &+ \frac{\eta_t}{\left|C_0\right|}(\left \| \nabla f^{0}(\omega_t) \right \|^2 + \nabla f^{0}(\omega_t)^\mathrm{T}\nabla f^{1}(\omega_t)) \notag
\end{align}
\noindent Note that $\theta_t=\angle(\nabla f^{0}(\omega_t), \nabla f^{1}(\omega_t))$. It reflects the degree of divergence between the inlier gradients and outlier gradients. A larger $\theta_t$ means a stronger rival between inliers and outliers, which may even drives the model parameters towards two opposite directions respectively. For clarity, we use a simplified notation $\nabla_{0} = \left\| \nabla f^{0}(\omega_t) \right\|$:
\begin{align}
&\frac{1}{\left|C_0\right|}f^{0}(\omega_t)-f^{0}(\omega_{t+1}) \ge \notag
\\ &\qquad-\frac{\eta_t^2 L}{2\left|C_0\right|} (\nabla_{0}^2 +\nabla_{1}^2 + 2\cos{\theta_t}\nabla_{0}\nabla_{1}) + \frac{\eta_t}{\left|C_0\right|}(\nabla_{0}^2 + \cos{\theta_t} \nabla_{0} \nabla_{1}) \label{lowerBound}
\end{align}
Now we get a lower bound of $f^{0}(\omega_t)-f^{0}(\omega_{t+1})$ with \eqref{applySmoothUpper}. With \eqref{applySmoothLower} and a similar procedure, we can derive a upper bound of $\frac{1}{\left|C_0\right|}f^{0}(\omega_t)-f^{0}(\omega_{t+1})$:
\begin{align}
&\frac{1}{\left|C_0\right|}f^{0}(\omega_t)-f^{0}(\omega_{t+1}) \le \notag
\\ &\qquad \frac{\eta_t^2 L}{2\left|C_0\right|} (\nabla_{0}^2 +\nabla_{1}^2 + 2\cos{\theta_t}\nabla_{0}\nabla_{1}) + \frac{\eta_t}{\left|C_0\right|}(\nabla_{0}^2 + \cos{\theta_t} \nabla_{0} \nabla_{1}) \label{upperBound}
\end{align}

\noindent \noindent Note that the previous formulas also apply to the other class $1-i$, since we assume that for each $i$, $f^i$ is $L-Smooth$. With assumption \ref{assumption2} and the inequation \eqref{lowerBound}, we have:
\\ \emph{For each class $i$,}
\begin{gather}
-\frac{\eta_t^2 L}{2} (\nabla_i^2 +\nabla_{1-i}^2 + 2\cos{\theta_t}\nabla_{0}\nabla_{1-i}) + \eta_t(\nabla_i^2 + \cos{\theta_t} \nabla_i \nabla_{1-i}) > 0 \notag
\end{gather}
\noindent Hence, 
\begin{gather}
\left\{
\begin{array}{l}
\eta_t L < \frac{2(\min(\nabla_{0}^2, \nabla_{1}^2) + \cos{\theta_t}\nabla_{0} \nabla_{1})}{\nabla_{0}^2 + 2\cos{\theta_t}\nabla_{0}\nabla_{1} + \nabla_{1}^2} \\
\theta_t<\cos^{-1}(-\frac{1}{r_t})
\end{array}
\right.
\end{gather}

From \eqref{lowerBound} and \eqref{upperBound}, we can get both upper and lower bounds of ${\triangle}^f_t = \frac{1}{\left|C_0\right|}(f^{0}(\omega_t)-f^{0}(\omega_{t+1}))-\frac{1}{\left|C_1\right|}(f^{1}(\omega_t)-f^{1}(\omega_{t+1}))$, which reflects the fluctuation of speed gap between two classes:
\begin{align}
   {\triangle}^f_t &\ge \frac{\eta_t \nabla^2_{1}}{\left|C_0\right|} ((r_t-R\cos\theta)^2-(R+1)^2)
\\ {\triangle}^f_t &\le \frac{\eta_t \nabla^2_{1}}{\left|C_0\right|} (r_t^2 + 2\cos\theta r_t + 1)
\end{align}
\end{proof}
In practice, speed gap usually floats between the upper and lower bounds. The difference value between the bounds is $ \frac{2\eta_t \nabla^2_{1}}{\left|C_0\right|}(R+1)(\cos\theta r_t+1)$, which reflects the magnitude of fluctuation of the speed gap.

